LoD-Loc: Aerial Visual Localization using LoD 3D Map with Neural Wireframe Alignment

We propose a new method named LoD-Loc for visual localization in the air. Unlike existing localization algorithms, LoD-Loc does not rely on complex 3D representations and can estimate the pose of an Unmanned Aerial Vehicle (UAV) using a Level-of-Detail (LoD) 3D map. LoD-Loc mainly achieves this goal by aligning the wireframe derived from the LoD projected model with that predicted by the neural network. Specifically, given a coarse pose provided by the UAV sensor, LoD-Loc hierarchically builds a cost volume for uniformly sampled pose hypotheses to describe pose probability distribution and select a pose with maximum probability. Each cost within this volume measures the degree of line alignment between projected and predicted wireframes. LoD-Loc also devises a 6-DoF pose optimization algorithm to refine the previous result with a differentiable Gaussian-Newton method. As no public dataset exists for the studied problem, we collect two datasets with map levels of LoD3.0 and LoD2.0, along with real RGB queries and ground-truth pose annotations. We benchmark our method and demonstrate that LoD-Loc achieves excellent performance, even surpassing current state-of-the-art methods that use textured 3D models for localization. The code and dataset are available at https://victorzoo.github.io/LoD-Loc.github.io/.

==> Tabel_rebuttal/Additianl_cost_compute.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{\textbf{Computational Cost Comparison.}} %We conducted test experiments on a single batch (Batch Size = 1) of images using the NVIDIA GeForce RTX 4090 device, and listed the average peak CUDA usage as well as the average inference time.}
\label{Tab:AddiBaeline_cost}
\begin{tabular}{cccc}
\toprule
\multicolumn{2}{c}{Method}       & Memory (Mb) & Time (s) \\ \midrule
\multirow{5}{*}{UAVD4L} & SPP    & 610         & 1.79     \\
                        & SIFT   & 443         & 1.85     \\
                        & LoFTR  & 2631        & 1.70     \\
                        & RoMA   & 5488        & 4.68    \\
                        & eLoFTR & 1650        & 1.06    \\ \hline
\multicolumn{2}{c}{ours}         & 4810        & 0.34     \\ 
\bottomrule
\end{tabular}
\end{table}

==> Tabel_rebuttal/Additional_Baseline.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{\textbf{Additional Experiments on Baseline over UAVD4L-LoD dataset.}} %We introduced different baselines, namely eLoFTR, RoMA and Explicit Line Alignment, to demonstrate comparisons with the latest methods. The Explicit Line Alignment method utilizes DeepLSD to extract explicit line segments and construct a distance field, and then refine the final pose based on the distance function. This highlights the necessity of using the feature extractor.}
\label{Tab:AddiBaeline}
\begin{tabularx}{\linewidth}{@{\extracolsep{\fill}}clcccccc}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{Method}}                 & \multicolumn{3}{c}{\textit{in-Traj.}}                     & \multicolumn{3}{c}{\textit{out-of-Traj.}}                 \\ \cmidrule(r){3-5} \cmidrule(r){6-8} 
\multicolumn{2}{c}{}                                        & 2m-2°           & 3m-3°           & 5m-5°           & 2m-2°           & 3m-3°           & 5m-5°           \\ \midrule
\multirow{2}{*}{\makecell[c]{UAVD4L\\ \textit{Mesh model}} }         & e-LoFTR          & 84.47          & 88.21          & 88.96         & 91.06          & 91.93          & 92.02          \\
                                         & RoMA          & 93.27 & 93.70          &  93.77          & 95.03          & 95.53          & 95.53          \\ \hline
\multirow{2}{*}{ \makecell[c]{CadLoc\\ \textit{LoD model}} } & e-LoFTR          & 0.37              & 0.87              & 1.31              & 0.41              & 0.78              & 1.37              \\
                                         & RoMA          & 2.18              & 2.87              & 3.68              & 6.93              & 8.76              & 10.40               \\ \hline
\multicolumn{2}{c}{\multirow{3}{*}{\makecell[c]{Explicit Line Alignment \\ \textit{LoD model} }}}              & \multirow{3}{*}{10.41}          & \multirow{3}{*}{16.21}          & \multirow{3}{*}{24.19}         & \multirow{3}{*}{6.93}          & \multirow{3}{*}{12.64}          & \multirow{3}{*}{21.62}          \\ \\
\\ \hline
\multirow{2}{*}{\makecell[c]{\textbf{Ours}\\ \textit{LoD model}}}       
                                         & \multirow{2}{*}{Full model}    & \multirow{2}{*}{84.41}          & \multirow{2}{*}{91.77} & \multirow{2}{*}{96.95} & \multirow{2}{*}{95.94} & \multirow{2}{*}{99.00} & \multirow{2}{*}{99.36} \\  \\
\bottomrule
\end{tabularx}
\end{table}

==> Tabel_rebuttal/Additional_Baseline_epfl.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{\textbf{Additional Experiments on Baseline over Swiss-EPFL dataset.}} %We introduced different baselines, namely eLoFTR, RoMA and Explicit Line Alignment, to demonstrate comparisons with the latest methods. The Explicit Line Alignment method is the same with Tab~\ref{Tab:AddiBaeline}.}
\label{Tab:AddiBaeline_epfl}
\begin{tabularx}{\linewidth}{@{\extracolsep{\fill}}clcccccc}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{Method}}                 & \multicolumn{3}{c}{\textit{in-Place.}}                     & \multicolumn{3}{c}{\textit{out-of-Place.}}                 \\ \cmidrule(r){3-5} \cmidrule(r){6-8} 
\multicolumn{2}{c}{}                                        & 2m-2°           & 3m-3°           & 5m-5°           & 2m-2°           & 3m-3°           & 5m-5°           \\ \midrule
\multirow{2}{*}{\makecell[c]{UAVD4L\\ \textit{Mesh model}} }         & e-LoFTR          & 37.64          & 60.96          & 76.40         & 81.53          & 91.03          & 93.93          \\
                                         & RoMA          & 45.98 & 66.77          &  80.73         & 89.18          & 98.68          & 98.94          \\ \hline
\multirow{2}{*}{ \makecell[c]{CadLoc\\ \textit{LoD model}} } & e-LoFTR          & 0              & 0.14              & 0.14              & 0              & 0              & 0.53              \\
                                         & RoMA          & 0.98              & 1.97              & 2.67             & 2.37              & 5.01              & 6.33               \\ \hline
\multicolumn{2}{c}{\multirow{3}{*}{\makecell[c]{Explicit Line Alignment \\ \textit{LoD model} }}}              & \multirow{3}{*}{11.37}          & \multirow{3}{*}{21.35}          & \multirow{3}{*}{33.57}         & \multirow{3}{*}{18.99}          & \multirow{3}{*}{31.39}          & \multirow{3}{*}{45.91}          \\ \\ \\ \hline
\multirow{2}{*}{\makecell[c]{\textbf{Ours}\\ \textit{LoD model}}}       
                                         & \multirow{2}{*}{Full model}    & \multirow{2}{*}{48.60}          & \multirow{2}{*}{65.31} & \multirow{2}{*}{79.78} & \multirow{2}{*}{37.73} & \multirow{2}{*}{57.26} & \multirow{2}{*}{77.57} \\ \\
\bottomrule
\end{tabularx}
\end{table}

==> Tabel_rebuttal/Additional_explict_align.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htp]
\centering
\caption{\textbf{Additional Experiments on Baseline over UAVD4L-LoD dataset.}}
\label{Tab:AddiBaeline}
\begin{tabularx}{\linewidth}{@{\extracolsep{\fill}}clcccccc}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{Method}}                 & \multicolumn{3}{c}{\textit{in-Traj.}}                     & \multicolumn{3}{c}{\textit{out-of-Traj.}}                 \\ \cmidrule(r){3-5} \cmidrule(r){6-8} 
\multicolumn{2}{c}{}                                        & 2m-2°           & 3m-3°           & 5m-5°           & 2m-2°           & 3m-3°           & 5m-5°           \\ \midrule
\multirow{2}{*}{\makecell[c]{Explicit\\ \textit{Alignment}} }         & \multirow{2}{*}{Method}          & \multirow{2}{*}{84.47          & \multirow{2}{*}{88.21          & \multirow{2}{*}{88.96         & \multirow{2}{*}{91.06          & \multirow{2}{*}{91.93          & \multirow{2}{*}{92.02          \\
\\
\bottomrule
\end{tabularx}
\end{table}

==> Tabel_rebuttal/inout_expla_old.tex <==

\begin{table}[h]
\centering
\small % Set font size to small (10pt)
\renewcommand{\arraystretch}{1.2} % Adjust row spacing
\begin{tabular}{p{1.6cm}p{2.2cm}p{2.8cm}p{2.2cm}p{3cm}}
\toprule
\textbf{Name} & \textbf{Capture device} & \textbf{Capture pitch angle} & \textbf{Capture height} & \textbf{Capture route} \\ \hline
\textit{in-Traj.} & DJI M300+H20t & 0\textdegree{} or 45\textdegree{} & 120m & Zig-zag flight on a selected region \\ 
\textit{out-of-Traj.} & DJI Mavic3 Pro & 30\textdegree{} $\sim$ 60\textdegree{} & 90m $\sim$ 150m & Manually controlled flight on the map \\ \bottomrule
\end{tabular}
\caption{\textbf{Key distinctions between \textit{in-Traj.} and \textit{out-of-Traj.}}.}
\end{table}


==> Table/Compare_JadeBay_intraj.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[hbtp]
\centering
\caption{The localization results on JadeBay in-traj.
  }
\label{Tab:JadeBay_inTraj}
\begin{tabular}{clcccccc}

\toprule
\multicolumn{2}{c}{\multirow{2}{*}{Method}}                         & \multicolumn{5}{c}{in-Traj.}                                                     & \multirow{2}{*}{Model Size} \\
\multicolumn{2}{c}{}                                                & 2m2°           & 3m3°           & 5m5°           & 10m7°          & 20m10°       &                                         \\ \midrule
\multicolumn{2}{c}{Sense Priors}                                    & 0              & 0              & 4.3            & 98.38          & \textbf{100} & /                                       \\ \hline
\multirow{6}{*}{UAVD4L}           & SIFT+NN          & 73.13          & 78.62          & 80.42          & 81.42          & 83.04        & \multirow{6}{*}{24.5 GB}             \\
                                                 & SPP+SPG          & \textbf{91.71} & \textbf{92.02} & \textbf{92.14} & 92.14          & 93.83        &                                         \\
                                                 & LoFTR            & 84.98          & 88.09          & 88.9           & 89.4           & 91.02        &                                         \\
                                                 & SOLD2            & 0              & 0              & 0              & 0              & 0.06         &                                         \\
                                                 & DeepLSD+Sold2    & 0              & 0              & 0.06           & 0.06           & 0.19         &                                         \\
                                                 & Deeplsd+GlueStick & 0              & 0              & 0.06           & 0.06           & 0.25         &                                         \\ \hline
\multirow{6}{*}{ImPerfect  model} & SIFT+NN          & 0              & 0              & 0              & 0              & 0            & \multirow{6}{*}{7.1 MB}                 \\
                                                 & SPP+SPG          & 0              & 0              & 0              & 0              & 0            &                                         \\
                                                 & LoFTR            & 0              & 0              & 0              & 0              & 0            &                                         \\
                                                 & SOLD2            & 0              & 0              & 0              & 0              & 0         &                                         \\
                                                 & DeepLSD+Sold2    & 0              & 0              & 0              & 0              & 0            &                                         \\
                                                 & Deeplsd+GlueStick & 0              & 0              & 0              & 0              & 0            &                                         \\ \hline
\multirow{3}{*}{OURS}                            & no ASR           & 24.63          & 60.22          & 86.28          & 99.38          & 99.81        & \multirow{3}{*}{\textbf{7.1 MB}}        \\
                                                 & no refine        & 51.93          & 77.37          & 89.53          & \textbf{99.63} & 99.69        &                                         \\
                                                 & \textbf{Full}    & 84.35          & \textbf{92.08} & \textbf{97.13} & 98.63          & 98.82        &                                         \\ 
\bottomrule
\end{tabular}
\end{table}

==> Table/Compare_JadeBay_outtraj.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htbp]
\centering
\caption{The localization results on JadeBay out-traj.
  }
\label{Tab:JadeBay_outTraj}
\begin{tabular}{clcccccc}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{Method}}          & \multicolumn{5}{c}{out-of-Traj.}                                                   & \multirow{2}{*}{Model Size} \\
\multicolumn{2}{c}{}                                 & 2m2°           & 3m3°           & 5m5°           & 10m7°          & 20m10°         &                                         \\ \midrule
\multicolumn{2}{c}{Sense   Priors}                   & 0              & 0              & 0.36           & 40.01          & 70.39          & /                                       \\ \hline
\multirow{6}{*}{UAVD4L}           & SIFT+NN          & 82.39          & 85.13          & 86.36          & 87             & 89.42          & \multirow{6}{*}{24.5 GB}             \\
                                  & SPP+SPG          & \textbf{93.43} & 93.7           & 93.8           & 93.98          & 96.99          &                                         \\
                                  & LoFTR            & 91.56          & 92.02          & 92.11          & 92.47          & 96.08          &                                         \\
                                  & SOLD2            & 0              & 0              & 0              & 0              & 0.14           &                                         \\
                                  & DeepLSD+Sold2    & 0              & 0              & 0              & 0              & 0.09           &                                         \\
                                  & Deeplsd+GlueStick & 0              & 0              & 0              & 0              & 0.09           &                                         \\ \hline
\multirow{6}{*}{ImPerfect  model} & SIFT+NN          & 0              & 0              & 0              & 0              & 0              & \multirow{6}{*}{7.1 MB}                 \\
                                  & SPP+SPG          & 0              & 0              & 0              & 0              & 0              &                                         \\
                                  & LoFTR            & 0              & 0              & 0              & 0              & 0              &                                         \\
                                  & SOLD2            & 0              & 0              & 0              & 0              & 0           &                                         \\
                                  & DeepLSD+Sold2    & 0              & 0              & 0              & 0              & 0           &                                         \\
                                  & Deeplsd+GlueStick & 0              & 0              & 0              & 0              & 0              &                                         \\ \hline
\multirow{3}{*}{OURS}             & no ASR           & 29.11          & 76.14          & 97.58          & 99.54          & 99.77          & \multirow{3}{*}{\textbf{7.1 MB}}        \\
                                  & no refine        & 72.76          & \textbf{97.67} & \textbf{99.59} & \textbf{99.59} & \textbf{99.68} &                                         \\
                                  & \textbf{Full}    & \textbf{95.39} & \textbf{98.91} & \textbf{99.22} & \textbf{99.27} & \textbf{99.27} &                                         \\ 
\bottomrule
\end{tabular}
\end{table}



==> Table/EPFL_outPlace.tex <==



==> section/abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
Current visual localization algorithms typically rely on complex 3D representations, such as Structure-from-Motion (SfM) results or textured mesh models, which are difficult to build, store, and maintain over time.
In this work, we introduce LoD-Loc, a novel localization framework that uses a Level-of-Detail (LoD) 3D city map to estimate the pose of a drone, providing a simple, accessible, and privacy-friendly scene representation.
LoD-Loc mainly estimates the 6-DoF pose of a query image by aligning the projected wireframe of the LoD model with the network-predicted building wireframe.
% LoD-Loc mainly estimates the 6-DoF pose of a query image by aligning network-predicted building wireframes and those projected from the LoD 3D map.
Given a prior pose, LoD-Loc hierarchically samples various pose hypotheses to build a pose cost volume, where each hypothesis computes a probability according to the LoD wireframe projection on the network-predicted wireframe map. The camera pose is inferred from the highest probability position in the volume. 
% Given a prior pose, LoD-Loc first determines a sampling range and generates a pose cost volume by projecting the wireframe onto a wireframe-predicted neural map to measure the alignment. The camera pose is inferred from the highest probability position in the volume. 
To ensure high accuracy and low memory usage, we determine the sampling space by estimating the uncertainty of the previous sampling step. 
% To ensure high accuracy and low memory usage, the cost volume is constructed progressively. The pose inference uncertainty of the previous level influences the sampling range of the current level.
We also devise a pose optimization algorithm to refine the result using a differentiable Gaussian-Newton method.
Moreover, we release two datasets with map levels of LoD3.0 and LoD2.0, along with real RGB queries with ground-truth pose annotation.
In these two datasets, LoD-Loc achieves excellent performance, even surpassing current state-of-the-art methods that use textured 3D models for localization. The code and dataset will be made available upon publication.

\keywords{Visual localization \and Pose estimation \and  Privacy-preserving localization}

\end{abstract}



==> section/dataset.tex <==
% \section{Datasets}
% \label{sec:data}

\begin{figure}[tb]
    \centering
	\includegraphics[width=1.0\linewidth]{Figure/Fig2.pdf}
	\caption{\textbf{Overview of datasets.} The left side shows the LoD models of the released data. The LoD2.0 model from Swiss-EPFL includes building height and roof information, while the LoD3.0 model from UAVD4L-LoD contains more detailed structural information such as building height, roof, and side pillars. The right side illustrates samples of query images, which consist of images captured by drones in various scenes.}
    \label{fig:data}
\end{figure}

The released datasets contain two distinct parts, named UAVD4L-LoD and Swiss-EPFL, providing LoD3.0 and LoD2.0 models, respectively. The UAVD4L-LoD dataset, which spans an area of 2.5 square kilometers, is derived from a semi-automatic process that generates a 3D LoD map based on the mesh model of the UAVD4L~\cite{wu2024uavd4l} dataset. This dataset encompasses a diverse array of architectural structures, including skyscrapers, villas, apartment complexes, educational institutions, and rural dwellings. The query images for this dataset are procured from two UAVs with real sensor data, specifically a DJI M300\cite{DJIM300} drone with an H20T\cite{DJIH20T} camera and a DJI Mavic3 Pro~\cite{Marvic3} drone. 
The Swiss-EPFL dataset, which covers an expansive area of 8.18 square kilometers, sources its LoD2.0 models from data made publicly accessible by the Swiss federal authorities~\cite{swisstopo1,swisstopo2,swisstopo3}. This dataset includes a variety of architectural styles, such as libraries, residential apartments, and stadiums. The query images for this dataset are obtained from the CrossLoc~\cite{yan2022crossloc} projects, captured using a DJI Phantom 4 RTK~\cite{Phatom4RTK} drone. We illuminate the 3D LoD maps and query images of these two datasets in Figure~\ref{fig:data}. More details on datasets can be found in Appendix~\ref{sec:detail_dataset},~\ref{sec:detail_UAV} and \ref{sec:detail_EPFL}.


% To facilitate further research in the field of LoD model localization, this research has prepared two UAV localization datasets, named JadeBay and Swiss-EPFL, owning LoD 3.0 model and LoD 2.0 model respectively. The JadeBay dataset comprises a georeferenced LoD 3.0 model, undistorted images with real sensor priors, and ground truth (GT) poses. The LoD 3.0 models are semi-automatically generated based on UAVD4L[] dataset, covering an area of $2.5$ square kilometers. The LoD 3.0 model includes various types of buildings such as high-level buildings, villas, residential buildings, school buildings, and rural houses. The Swiss-EPFL dataset consists of a georeferenced LoD 2.0 model, undistorted images with randomly generated priors, and GT poses. The LoD 2.0 models are sourced from publicly available data provided by the Swiss federal authorities, covering a total area of $8.18$ square kilometers. This area encompasses buildings of different styles, including residential buildings and school structures.



